Scalar fields in the nonsymmetric Kaluza-Klein (Jordan-Thiry) theory

In this paper we construct the Nonsymmetric Jordan-Thiry Theory unifying N.G.T., the Yang-Mills' field, the Higgs' fields and scalar forces in a geometric manner. In this way we get masses from higher dimensions. We discuss spontaneous symmetry breaking, the Higgs' mechanism and a mass generation in the theory. The scalar field (as in the classical Jordan-Thiry Theory) is connected to the effective gravitational constant. This field is massive and has Yukawa-type behaviour. We derive the equation of motion for a test particle from conservation laws in the hydrodynamic limit. We consider a truncation procedure for a tower of massive scalar fields using Friedrichs' theory and an approximation procedure for the lagrangian involving Higgs' field. The geodetic equations on the Jordan-Thiry manifold are considered with an emphasis to terms involving Higgs' field. We consider also field equations in linear approximation. We consider a dynamics of Higgs' field in the framework of cosmological models involving the scalar field. The scalar field plays here a role of a quintessence field. We consider phase transition in cosmological models of the second and the first order. We consider a warp factor known from some modern approaches. We consider a toy model of a time-machine. We consider a mass of a quintessence particle, various properties of a quintessence field. We calculate a speed of sound in a quintessence and fluctuations of a quintessence caused by primordial metric fluctuations.

==> linie.tex <==
\newdimen\jedn
\catcode`@=11
\newcount\@multicnt
\newdimen\@xdim
\newdimen\@ydim
\long\def\put(#1,#2)#3{\raise#2\jedn\hbox to\z@{\kern#1\jedn#3\hss}\ignorespaces}
\def\linia(#1,#2)(#3,#4){\put(#1,#2){\special{em:moveto}}%
    \put(#3,#4){\special{em:lineto}}}
\def\grub#1 {\special{em:linewidth #1}}
\long\def\multi(#1,#2)(#3,#4)#5#6{\@multicnt=#5\relax
\@xdim=#1\jedn
\@ydim=#2\jedn
\loop\ifnum \@multicnt>\z@
\raise\@ydim\hbox to\z@{\kern\@xdim\hbox{#6}\hss}\advance\@multicnt by-1 \advance\@xdim
#3\jedn\advance\@ydim #4\jedn \repeat \ignorespaces}
\def\MT #1 #2 {\put(#1,#2){\special{em:moveto}}}
\def\LT #1 #2 {\put(#1,#2){\special{em:lineto}}}
\catcode`@=12
\grub0.4pt
\newdimen\sz
\sz=1truemm
\jedn=\sz
\long\def\cput(#1,#2,#3){\put(#1,#2){\hbox to0pt{\hss$#3$\hss}}}
\long\def\rput(#1,#2,#3){\put(#1,#2){\hbox to0pt{$#3$\hss}}}
\long\def\lput(#1,#2,#3){\put(#1,#2){\hbox to0pt{\hss$#3$}}}
\def\str(#1,#2)(#3,#4)(#5,#6){\MT #3 #4 \LT #1 #2 \LT #5 #6 }
\endinput

